Distributionally Robust Optimization with Probabilistic Group

Modern machine learning models may be susceptible to learning spurious correlations that hold on average but not for the atypical group of samples. To address the problem, previous approaches minimize the empirical worst-group risk. Despite the promise, they often assume that each sample belongs to one and only one group, which does not allow expressing the uncertainty in group labeling. In this paper, we propose a novel framework PG-DRO, which explores the idea of probabilistic group membership for distributionally robust optimization. Key to our framework, we consider soft group membership instead of hard group annotations. The group probabilities can be flexibly generated using either supervised learning or zero-shot approaches. Our framework accommodates samples with group membership ambiguity, offering stronger flexibility and generality than the prior art. We comprehensively evaluate PG-DRO on both image classification and natural language processing benchmarks, establishing superior performance

==> tables/analysis_nlp.tex <==
\begin{table*}[t]
\caption{\small Comparison of average and worst-group test accuracies for combinations of different group labeling approach and robust training methods when evaluated on NLP datasets: MultiNLI~\cite{williamsnli} \& CivilComments-WILDS~\cite{borkancivil, koh2021wilds}. Results (mean and std) of our proposed methods are estimated over 3 random seeds for consistency. Best performing results for each pseudo labeling approach are marked in \textbf{bold}.} 
\label{tab:analysis_nlp_table}
\small
\centering
 \begin{tabular}{l ccccc}
\toprule
  \multirow{2}{2.5cm}{\textbf{Method}} &  \multirow{2}{*}{\centering Dataset with group label} & \multicolumn{2}{c}{\centering \textbf{MultiNLI}} & \multicolumn{2}{c}{\centering \textbf{CivilComments-WILDS}}\\ \cmidrule{3-6}
& &  Avg. Acc & Worst Group Acc & Avg. Acc &  Worst Group Acc \\
 \midrule
ERM & None & 82.6 & 66.4 & 92.6 & 58.4\\
\midrule
 G-DRO~\cite{sagawa2019distributionally} & train \& val. set & 81.4$_{\pm{0.1}}$ & 77.5$_{\pm{1.2}}$ & 87.7$_{\pm{0.6}}$ & 69.1$_{\pm{0.8}}$\\
\midrule
SSA~\cite{nam2022spread} & val. set & 79.9$_{\pm{0.9}}$ & 76.6$_{\pm{0.7}}$ & 88.2$_{\pm{2.0}}$ & 69.9$_{\pm{2.0}}$ \\
PG-DRO (Ours) & val. set & 80.8$_{\pm{0.3}}$ & \textbf{78.6}$_{\pm{0.6}}$ & 87.6$_{\pm{1.9}}$ & \textbf{79.5}$_{\pm{2.1}}$ \\
\midrule
 SSA~\cite{nam2022spread}  & $5\%$ of val. set & 80.4$_{\pm{0.6}}$ & 76.5$_{\pm{1.9}}$ & 89.1$_{\pm{1.1}}$ & 69.5$_{\pm{1.2}}$ \\
PG-DRO (Ours) & $5\%$ of val. set & 80.5$_{\pm{0.4}}$ & \textbf{78.4}$_{\pm{0.9}}$ & 87.5$_{\pm{1.4}}$ & \textbf{79.3}$_{\pm{1.5}}$ \\
\bottomrule

\end{tabular}
\end{table*}























































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































==> tables/clip_arch_ablations.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\begin{table}[t]
\caption{Comparison of average and worst-group test accuracies when using different architectures architectures as image encoder in pretrained CLIP model for generating pseudo labels.}
\label{tab:clip_arch_ablations}
\small
\centering
 \begin{tabular}{l c p{1.4cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{1.4cm}  >{\centering\arraybackslash}p{1cm}}
\toprule
 \multirow{2}{2.5cm}{Method} & \multirow{2}{3cm}{ \centering Architecture \\ (Image Encoder)} & \multicolumn{2}{c}{\centering Waterbirds} & \multicolumn{2}{c}{\centering CelebA}\\ \cmidrule{3-6}
 & &  Avg. & Worst Group & Avg. &  Worst Group \\
 \midrule
 \multirow{4}{*}{Hard + Group-DRO} & ViT-L/14 & 91.2 & 87.5 & 93.2 & 87.8 \\
& ViT-B/32 & 0 & 0 & 0 & 0 \\
& ViT-B/16 & 0 & 0 & 0 & 0 \\
& RN50x64 & 0 & 0 & 0 & 0 \\
\midrule
\multirow{4}{*}{Soft + PGDRO} & ViT-L/14 & 91.7 & 89.3 & 92.8 & 88.8 \\
& ViT-B/32 & 0 & 0 & 0 & 0 \\
& ViT-B/16 & 0 & 0 & 0 & 0 \\
& RN50x64 & 0 & 0 & 0 & 0 \\
 \bottomrule
 \end{tabular}
\end{table}
